DecAF: Joint Decoding of Answers and Logical Forms for Question Answering over Knowledge Bases

Question answering over knowledge bases (KBs) aims to answer natural language questions with factual information such as entities and relations in KBs. Previous methods either generate logical forms that can be executed over KBs to obtain final answers or predict answers directly. Empirical results show that the former often produces more accurate answers, but it suffers from non-execution issues due to potential syntactic and semantic errors in the generated logical forms. In this work, we propose a novel framework DecAF that jointly generates both logical forms and direct answers, and then combines the merits of them to get the final answers. Moreover, different from most of the previous methods, DecAF is based on simple free-text retrieval without relying on any entity linking tools -- this simplification eases its adaptation to different datasets. DecAF achieves new state-of-the-art accuracy on WebQSP, FreebaseQA, and GrailQA benchmarks, while getting competitive results on the ComplexWebQuestions benchmark.

==> rebuttal.tex <==
Paper Link: https://www.overleaf.com/8353453713pbjfwdgpnfcj
Review Link: https://openreview.net/forum?id=XHc5zRPxqV9

General Response:

We thank all the reviewers for their precious time and insightful comments. We appreciate that the reviewers recognize our work as well-motivated (Reviewer ZmkY, 9YKE), empirically effective (Reviewer ZmkY, Azh2, 9YKE), and well-written (Reviewer ZmkY, Azh2, 9YKE). We want to summarize the novel contributions of our work:
We are the first to propose a unified KBQA framework that combines the merits of both semantic parsing and direct question answering. 
We remove the entity linking efforts and use text-based retrieval to enhance the adaptability of our model to new domains.
Our method achieves new state-of-the-arts on 3 benchmark datasets, with significant improvements in F1 scores over WebQSP (2.3%) and FreebaseQA (15.7%), and 1st rank on the GrailQA leaderboard.
To improve the paper's quality, we respond to the reviewers’ comments by making the following revisions (marked in blue) to the paper:
We add more analysis on what type of questions can logical form or answer generation perform better in Appendix A.5, as suggested by Reviewer ZmkY, Azh2, and 9YKE. We show that compared to semantic parsing, direct-answer generation is preferable when the number of relations in the logical form increases and the number of total answers decreases. We also show that direct-answer generation is more advantageous on the zero-shot questions rather than I.I.D and compositional ones.
We add the experiment results of other types of combination methods in Appendix A.4, as suggested by Reviewer ZmkY. We show that our model outperforms the combination of the strongest semantic parsing baselines and direct-answer generation methods.
We add the results of the oracle combination method over LF-executed answers and generated answers in Appendix A.6, as suggested by Reviewer ZmkY. We show that the oracle combination has better performances compared to our original combination, but not that much (<= 3 points improvement), which indicates that our current combination method (first LF execution then direct generation) is a simple but very effective choice.
Response to Reviewer ZmkY (Score 5):

We appreciate the in-depth questions and suggestions given by the reviewer. 

We have provided our responses below.

It only appears to be a step beyond ensembling, where the systems being ensembled are just two routes to answer from the same reader.

One reader can produce both logical form and answer, the answers come from different sauces, and they can be further combined.

The ablation analyses, unfortunately, don't yield any interesting insights.

We’ve added additional analysis in Appendix XXX. Please kindly refer to our general response. 

it would be nice to gain insight on the questions for which we can get answers via the direct generation method but not via logical form execution

We directly compare the LF-executed answers and direct-generated answers on different question categories of the GrailQA (dev) dataset. The table below shows 4 different comparison results, where we calculate the percentages of questions that they perform equally well, LF better, Answer better and they both have the F1 score of 0. We see that direct-answer generation has more advantages on the zero-shot questions (15.3%) compared to I.I.D (4.4%) and compositional (6.7%) ones. This also corresponds to the second example in Table 11 where we see that for zero-shot questions with schemas unseen during training, generating the correct logical forms containing the schemas can be very difficult. 



Overall
 I.I.D.
Compositional
Zero-Shot
LF better
33.0%
40.6%
48.4%
23.4%
Answer better
10.8%
4.4%
6.7%
15.3%
Equal F1
39.4%
47.2%
28.1%
40.8%
Zero F1
16.7%
7.8%
16.8%
20.5%


We also conduct a similar analysis based on the number of relations in the ground-truth logical form of each question. The table below shows that the direct-answer generation has more advantages when the number of relations increases (7.3% -> 18.8% -> 29.1%), where the logical forms become more complicated and harder to generate.

# Relation
1
 2
>= 3
# Question
4950
1528
285
LF better
33.1%
35.7%
17.9%
Answer better
7.3%
18.8%
29.1%
Equal F1
46.4%
22.6%
9.1%
Zero F1
13.3%
22.8%
43.9%



Other types of combinations: Would it be useful to think about other choices of two methods for combining answers? 

We select two published best semantic-parsing baseline methods ArcaneQA and RnG-KBQA, and combine them with our direct-answer generation results. That is, if their generated logical forms are not executable, we use the directly generated answers by DecAF as the final answer. We also combine these two baseline methods: if the logical forms generated by one of them are not executable, use the logical forms generated by the other method. 
As shown in the Table below where F1 scores are reported, we see that they still underperform our DecAF method. After looking at their results in more detail, we find that for ArcaneQA and RnG-KBQA, very few questions have non-executable logical forms. For ArcaneQA, the corresponding question percentages are 0.7% and 1.4% on WebQSP and GrailQA. For RnG-KBQA, they are 1.8% and 0%. For our model DecAF (FiD-large), they are 11.3% and 15.8%. The reason is that ArcaneQA uses constrained decoding and RnG-KBQA uses logical form enumeration to increase the execution rate of their generated logical forms. But a high execution rate does not mean high accuracy. We argue that for some questions (like zero-shot and multi-relational questions as mentioned in Question 1), instead of forcing the model to generate executable logical forms, switching to direct-answer generation is a better choice.

Model
Combination Type
WebQSP
GrailQA (dev)
ArcaneQA
None
75.6
76.9
ArcaneQA + DecAF (FiD-large, Answer Only)
LF + Answer
75.8
77.4
ArcaneQA + DecAF (FiD-3B, Answer Only)
LF + Answer
75.8
77.5
ArcaneQA + RnG-KBQA
LF + LF
76.0
77.0
RnG-KBQA
None
76.2 
77.1
RnG-KBQA + DecAF (FiD-large, Answer Only)
LF + Answer
76.9
77.1
RnG-KBQA + DecAF (FiD-3B, Answer Only)
LF + Answer
77.0
77.1
RnG-KBQA + ArcaneQA
LF + LF
77.2
77.1
DecAF (FiD-large)
LF + Answer
77.1
78.7
DecAF (FiD-3B)
LF + Answer
78.8
81.4



Oracle experiments: It would be useful to know what the upper-bound performance you can hope for if you allowed an oracle to choose between the top answer from the direct and execution based method? 

Good suggestion. We conduct the oracle combination by selecting the better answer from direct generation and LF-execution based on its F1 score with the ground-truth answer. We report the oracle results below compared to the original results. We see that the oracle combination does have better performance compared to our original model, but not that much (<= 3 points improvement), which indicates that our current combination method (first LF execution then direct generation) is a simple but very effective choice.

Model
WebQSP
CWQ
GrailQA (dev)
F1
Hits@1
F1
DecAF (FiD-large)
77.1
68.1
78.7
DecAF (FiD-large, Oracle)
79.6
70.1
80.7
DecAF (FiD-3B)
78.8
70.4
81.4
DecAF (FiD-3B, Oracle)
81.8
72.1
83.6



Question difficulty: It would be useful to know the performance of the direct answer generation accuracy on the set of questions for which the logical form based execution fails. 

We collect, in the table below, the direct answer generation accuracy on the set of questions where the generated logical forms are not executable. From the result, we observe that the performance of direct-answer generation for the data subset for non-executable LF is much lower than the overall evaluation dataset (19.6% F1 drop in WebQSP, 13% Hit@1 drop in CWQ and 14.7 F1 drop in GrailQA). Therefore, it shows that the set of questions for which the logical form based execution fails is also difficult for direct answer generation.

Question Type
WebQSP
CWQ
GrailQA (dev)
F1
Hits@1
F1
Overall
49.8
50.5 
54.7
Non-executable LF 
30.2
37.5 
40.0


Response to Reviewer 9YKE (Score 5): 

Thanks for your questions and suggestions. We have provided our responses below.

The combination mechanism of logical forms and direct answers lacks novelty.

The collaboration between logical forms and direct answers can be analyzed more in-depth.

In addition to considering the executability of logical forms, on what kinds of questions can each method demonstrate its unique merits? And how does the complementary effect form?

[Copy the answer to Question 1 for Reviewer ZmKY. add the following response]:

We further conduct analysis based on the number of ground-truth answers to each question. The table below shows that logical-form generation has more advantages when the number of answers increases (from 14.8% to 82.7%). This is reasonable since the difficulty of logical form generation is not necessarily correlated with the number of answers while this is not the case for direct-answer generation.

# Answer
1
 2-4
5-9
10+
# Question
4718
1114
352
579
LF better
14.8%
71.4%
74.4%
82.7%
Answer better
10.6%
13.0%
12.2%
8.1%
Equal F1
56.2%
1.0%
0.3%
0%
Zero F1
18.4%
14.6%
13.1%
9.2%


Response to Reviewer Azh2 (Score 6): 

Thanks for your questions and suggestions. We have provided our responses below.

intuition behind why training a model to produce both logical forms and direct answers is expected to work better? Is it because for some questions it is easier to predict the logical forms and for some it is easier to directly decode the answer and hence it is best to combine both?

Correct. We conduct more in-depth analysis below.
[Copy the answer to Question 1 for Reviewer 9YKE]


These datasets contain many questions which have multiple answers. How do you handle that during training and testing? Is the direct-decode model trained to produce all answers?

The current direct-decode model only generates a single answer instead of multiple answers together. During training, we randomly sample an answer as the training target for each training step. During testing, we choose the top-1 generated answer using beam search. We also tried to generate multiple answers as discussed in Appendix A.3, where we find that it can improve the performance of direct-answer generation, but the final performance after combination with logical-form generation is not improved. We think the reason is that the performance improvement of multi-answer generation comes from the questions that logical forms can also perform very well. We leave the exploration of more advanced multi-answer generation methods as future work.

Response to Reviewer B5YN (Score 8):

Thanks for your positive comments. We have provided our response below.

LLMs (in this case T5) are pre-trained on well-formed sentences. However, the retrieved subgraph is the form of <head relation tail> which is not well-formed. How will this affect its representation?

Although T5 is pre-trained mainly on well-formed sentences, we found that it can capture the information of the retrieved subgraphs very well. As shown in Figure 2 on Page 9, increasing the number of retrieved passages can significantly improve the model performance, which demonstrates that T5 is effectively leveraging the information from those passages. One recent paper UDT-QA [1] also conducts an interesting experiment, where it verbalizes KGs by transforming triplets into well-formed sentences, but the performance improvement is not that significant as shown in Table 2 of the UDT-QA paper. This also indicates that LLMs can capture the information of text that is not well-formed, at least in the supervised setting where training data from downstream tasks are provided. It would be interesting to study this at the zero-shot or few-shot settings.

[1] Ma, Kaixin, et al. "Open Domain Question Answering with A Unified Knowledge Interface." Proceedings of the 60th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers). 2022.

